Indexing Multimodal Language Models for Large-scale Image Retrieval

Multimodal Large Language Models (MLLMs) have demonstrated strong cross-modal reasoning capabilities, yet their potential for vision-only tasks remains underexplored. We investigate MLLMs as training-free similarity estimators for instance-level image-to-image retrieval. Our approach prompts the model with paired images and converts next-token probabilities into similarity scores, enabling zero-shot re-ranking within large-scale retrieval pipelines. This design avoids specialized architectures and fine-tuning, leveraging the rich visual discrimination learned during multimodal pre-training. We address scalability by combining MLLMs with memory-efficient indexing and top-$k$ candidate re-ranking. Experiments across diverse benchmarks show that MLLMs outperform task-specific re-rankers outside their native domains and exhibit superior robustness to clutter, occlusion, and small objects. Despite strong results, we identify failure modes under severe appearance changes, highlighting opportunities for future research. Our findings position MLLMs as a promising alternative for open-world large-scale image retrieval.

==> fig/llm_vs_global_vs_ames.tex <==
\scriptsize
\begin{tabular}{@{\hspace{-2pt}}c@{\hspace{1pt}}c@{\hspace{12pt}}c@{\hspace{1pt}}c@{\hspace{12pt}}c@{\hspace{1pt}}c@{\hspace{12pt}}c@{\hspace{1pt}}c@{\hspace{12pt}}c@{\hspace{1pt}}c@{\hspace{-2pt}}}

% First case 
\multicolumn{10}{c}{\textbf{global \vs Qwen~~~---~~~Qwen outperforms~~~---~~~global $\rightarrow$ Qwen}} \\[0pt]
\multicolumn{2}{c}{$988 \rightarrow 0$} &
\multicolumn{2}{c}{$991 \rightarrow 4$} &
\multicolumn{2}{c}{$977 \rightarrow 14$} &
\multicolumn{2}{c}{$947 \rightarrow 8$} &
\multicolumn{2}{c}{$941 \rightarrow 4$} \\[0pt]
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm1_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm1_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm2_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm2_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm3_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm3_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm4_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm4_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm5_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm5_d.jpg} \\[0pt]
\multicolumn{2}{c}{$917 \rightarrow 3$} &
\multicolumn{2}{c}{$924 \rightarrow 11$} &
\multicolumn{2}{c}{$967 \rightarrow 87$} &
\multicolumn{2}{c}{$901 \rightarrow 0$} &
\multicolumn{2}{c}{$890 \rightarrow 0$} \\[0pt]
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm6_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm6_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm7_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm7_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm8_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm8_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm9_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm9_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm10_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/llm10_d.jpg} \\[2pt]


% Second case 
\multicolumn{10}{c}{\textbf{global \vs Qwen~~~---~~~global outperforms~~~---~~~Qwen $\rightarrow$ global}} \\[0pt]
\multicolumn{2}{c}{$963 \rightarrow 140$} &
\multicolumn{2}{c}{$808 \rightarrow 4$} &
\multicolumn{2}{c}{$764 \rightarrow 85$} &
\multicolumn{2}{c}{$310 \rightarrow 100$} &
\multicolumn{2}{c}{$218 \rightarrow 4$} \\[0pt]
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global1_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global1_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global2_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global2_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global3_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global3_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global4_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global4_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global5_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global5_d.jpg} \\[0pt]
\multicolumn{2}{c}{$250 \rightarrow 0$} &
\multicolumn{2}{c}{$189 \rightarrow 12$} &
\multicolumn{2}{c}{$200 \rightarrow 4$} &
\multicolumn{2}{c}{$124 \rightarrow 7$} &
\multicolumn{2}{c}{$122 \rightarrow 1$} \\[0pt]
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global6_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global6_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global7_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global7_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global8_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global8_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global9_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global9_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global10_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_global/global10_d.jpg} \\[2pt]


% Third case 
\multicolumn{10}{c}{\textbf{AMES \vs Qwen~~~---~~~Qwen outperforms~~~---~~~AMES $\rightarrow$ Qwen}} \\[0pt]
\multicolumn{2}{c}{$859 \rightarrow 0$} &
\multicolumn{2}{c}{$873 \rightarrow 3$} &
\multicolumn{2}{c}{$926 \rightarrow 0$} &
\multicolumn{2}{c}{$874 \rightarrow 15$} &
\multicolumn{2}{c}{$797 \rightarrow 0$} \\[0pt] 
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm1_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm1_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm2_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm2_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm3_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm3_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm4_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm4_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm5_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm5_d.jpg} \\[0pt]
\multicolumn{2}{c}{$741 \rightarrow 4$} &
\multicolumn{2}{c}{$759 \rightarrow 26$} &
\multicolumn{2}{c}{$721 \rightarrow 1$} &
\multicolumn{2}{c}{$753 \rightarrow 25$} &
\multicolumn{2}{c}{$699 \rightarrow 0$} \\[0pt]
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm6_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm6_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm7_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm7_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm8_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm8_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm9_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm9_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm10_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/llm10_d.jpg} \\[2pt]

% Fourth case 
\multicolumn{10}{c}{\textbf{AMES \vs Qwen~~~---~~~AMES outperforms~~~---~~~Qwen $\rightarrow$ AMES}} \\[0pt]
\multicolumn{2}{c}{$523 \rightarrow 0$} &
\multicolumn{2}{c}{$536 \rightarrow 16$} &
\multicolumn{2}{c}{$616 \rightarrow 113$} &
\multicolumn{2}{c}{$456 \rightarrow 58$} &
\multicolumn{2}{c}{$365 \rightarrow 0$} \\[0pt]
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames1_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames1_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames2_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames2_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames3_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames3_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames4_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames4_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames5_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames5_d.jpg} \\
\multicolumn{2}{c}{$453 \rightarrow 93$} &
\multicolumn{2}{c}{$219 \rightarrow 16$} &
\multicolumn{2}{c}{$210 \rightarrow 14$} &
\multicolumn{2}{c}{$434 \rightarrow 245$} &
\multicolumn{2}{c}{$633 \rightarrow 447$} \\[0pt]
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames6_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames6_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames7_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames7_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames8_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames8_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames9_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames9_d.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames10_q.jpg} &
\includegraphics[height=1.4cm,width=1.4cm]{fig/llm_vs_global_ames/llm_vs_ames/ames10_d.jpg} \\


\end{tabular}


==> preamble.tex <==
% 
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\usepackage{xcolor}
\usepackage{array}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage[export]{adjustbox} % required for 'clip'


==> tab/sota_reb.tex <==
\newcolumntype{C}{>{\centering\arraybackslash}p{3.2em}}
\renewcommand{\arraystretch}{.9}
\setlength\tabcolsep{1pt}
\scriptsize
\begin{tabular}{lCCCCCCC}
\toprule
\textbf{Method} & \textbf{\ilias} & \textbf{INST} & $\cR$\textbf{OP} & \textbf{\prodonem} & \textbf{iNat} \\ \midrule

~~\textbf{No re-rank}                 & 26.5 & 82.2 & 67.5 & 52.2 & 55.5  \\
~~\textbf{AMES}                       & 34.2 & 85.1 & \textbf{82.1} & 54.1 & 54.6 \\ 
~~\textbf{LamRA}                      & 39.4 & 89.1 & & 62.7 & \textbf{61.2} \\
~~\textbf{Qwen}                       & 32.8 & 89.1 & 64.5 & 62.4 & 59.4 \\
\hline
\rowcolor{lightgray}
~~\textbf{LamRA}                      & 41.2 & 90.5 & 67.9 & 62.2 & \textbf{62.9} \\
\rowcolor{lightgray}
~~\textbf{Qwen}                       & \textbf{41.7} & \textbf{90.7} & 71.1 & \textbf{64.4} & 61.2 \\

\bottomrule
\end{tabular}
